CompArt: Operationalizing Aesthetic Alignment in Text-to-Image Generation via Principles of Art

Text-to-Image (T2I) diffusion models have made rapid progress on semantic alignment (generating what is described in the prompt), yet users still lack reliable control over aesthetic composition (how visual elements are put together). Prior work often treats aesthetics as a single, preference-driven notion (e.g., "high quality", "detailed", "breathtaking"), which does not map cleanly to compositional intent. We propose Aesthetic Alignment: aligning generated images to explicit, user-specified compositional constraints. We operationalize these constraints using the Principles of Art (PoA)-e.g., Balance, Rhythm, and Emphasis-commonly used in art education to describe composition. To support this task, we introduce CompArt, a dataset of 80,032 WikiArt images augmented with captions and PoA analyses produced by a multimodal LLM under structured prompting. We further propose ArtDapter, a lightweight and disentangled adapter that enables steering a pretrained T2I model along 10 PoA dimensions while retaining the base model's semantic capability. Experiments on CompArt show improved adherence to PoA controls over strong baselines under a dual evaluation protocol.

==> fig/compart_qualitative_issues.tex <==
\begin{figure}[htbp]
    \centering
    \scriptsize
        \begin{subfigure}{0.21\textwidth}
            \centering
            \includegraphics[height=3.5cm]{assets/compart_qualitative/orest-kiprensky_portrait-of-a-military-doctor-1812.jpg}
            \caption{}
            \label{fig:orest-kiprensky_portrait-of-a-military-doctor-1812}
            \parbox[t]{0.9\textwidth}{Symmetric balance is evident in the composition, with the man's figure centrally placed and evenly distributed visual weight on both sides, creating a sense of stability and order.}
        \end{subfigure}%
        \begin{subfigure}{0.21\textwidth}
            \centering
            \includegraphics[height=3.5cm]{assets/compart_qualitative/francisco-goya_the-duke-of-osuna-and-his-family-1788.jpg}
            \caption{}
            \label{fig:francisco-goya_the-duke-of-osuna-and-his-family-1788}
            \parbox[t]{0.9\textwidth}{Symmetric balance is evident in the composition, with the man and woman positioned centrally and the children symmetrically arranged around them, creating a sense of stability and order.}
        \end{subfigure}%
        \begin{subfigure}{0.21\textwidth}
            \centering
            \includegraphics[height=3.5cm]{assets/compart_qualitative/giovanni-bellini_madonna-and-child-1490.jpg}
            \caption{}
            \label{fig:giovanni-bellini_madonna-and-child-1490}
            \parbox[t]{0.9\textwidth}{Symmetric balance is evident in the composition, with the woman and child centrally placed and mirrored on either side, creating a sense of stability and harmony.}
        \end{subfigure}%
        \begin{subfigure}{0.16\textwidth}
            \centering
            \includegraphics[height=3.5cm]{assets/compart_qualitative/joshua-reynolds_frederick-howard-5th-earl-of-carlisle.jpg}
            \caption{}
            \label{fig:joshua-reynolds_frederick-howard-5th-earl-of-carlisle}
            \parbox[t]{0.9\textwidth}{Asymmetric balance is evident in the composition, with the young man positioned to the left and the architectural elements providing visual weight on the right. This balance creates a dynamic and engaging visual experience.}
        \end{subfigure}%
        \begin{subfigure}{0.21\textwidth}
            \centering
            \includegraphics[height=3.5cm]{assets/compart_qualitative/lorenzo-lotto_allegory-of-chastity-1505.jpg}
            \caption{}
            \label{fig:compart_qualitative/lorenzo-lotto_allegory-of-chastity-1505}
            \parbox[t]{0.9\textwidth}{Asymmetric balance is evident in the composition, with the reclining woman on the right side balanced by the cherub and trees on the left, creating a harmonious yet dynamic visual equilibrium.}
        \end{subfigure}%
        \vspace{1em}
        \begin{subfigure}{0.16\textwidth}
            \centering
            \includegraphics[height=2.5cm]{assets/compart_qualitative/odilon-redon_the-angel-of-destiny.jpg}
            \caption{}
            \label{fig:compart_qualitative/odilon-redon_the-angel-of-destiny}
            \parbox[t]{0.9\textwidth}{Asymmetric balance is evident in the composition, with the figure and boat placed off-center to the left, counterbalanced by the vast empty space on the right. This creates a sense of unease and tension.}
        \end{subfigure}%
        \begin{subfigure}{0.26\textwidth}
            \centering
            \includegraphics[height=2.5cm]{assets/compart_qualitative/boris-kustodiev_in-the-box-1912.jpg}
            \caption{}
            \label{fig:boris-kustodiev_in-the-box-1912}
            \parbox[t]{0.9\textwidth}{Asymmetric balance is evident in the composition, with the three individuals on the left side and the vibrant stage on the right side, creating a balanced yet dynamic visual weight.}
        \end{subfigure}%
        \begin{subfigure}{0.26\textwidth}
            \centering
            \includegraphics[height=2.5cm]{assets/compart_qualitative/bartolome-esteban-murillo_adoration-of-the-shepherds-1.jpg} % 
            \caption{}
            \label{fig:bartolome-esteban-murillo_adoration-of-the-shepherds-1}
            \parbox[t]{0.9\textwidth}{Asymmetric balance is evident in the composition, with the figures on the left side balanced by the animals and the angel on the right, creating a dynamic yet stable arrangement.}
        \end{subfigure}%
        \begin{subfigure}{0.16\textwidth}
            \centering
            \includegraphics[height=2.5cm]{assets/compart_qualitative/gustav-klimt_roses-under-the-tree.jpg}
            \caption{}
            \label{fig:gustav-klimt_roses-under-the-tree}
            \parbox[t]{0.9\textwidth}{Asymmetric balance is evident in the composition, with the dense tree canopy on the left side balanced by the patches of white and pink flowers on the right side, creating a sense of stability and equilibrium.}
        \end{subfigure}%
        \begin{subfigure}{0.16\textwidth}
            \centering
            \includegraphics[height=2.5cm]{assets/compart_qualitative/koloman-moser_picture-book-for-the-niece-of-ditha-mautner-von-markhof-1904-3.jpg}
            \caption{}
            \label{fig:koloman-moser_picture-book-for-the-niece-of-ditha-mautner-von-markhof-1904-3}
            \parbox[t]{0.9\textwidth}{Asymmetric balance is evident in the composition with the seven dogs on the right side and the four birds on the left side, creating a visual equilibrium despite the different elements.}
        \end{subfigure}
    \caption{Issues observed in CompArt PoA annotations on the principle of Balance.}
    \label{fig:compart-qualitative-issues}
\end{figure}

==> fig/compose_wise.tex <==
\begin{figure}[H]
    \scriptsize
    \centering
    \setlength{\columnsep}{1em}
    \begin{multicols}{3}
        \begin{subfigure}{\linewidth}
        \includegraphics[width=\textwidth]{assets/artdapted_qualitative/combined_lawren-harris_afternoon-sun-lake-superior-1924.jpg}
        \caption{}
        \parbox[t]{\linewidth}{
        \textbf{Prompt:} Landscape with a view of a body of water, islands, and distant hills under a sky with orange clouds, with tall, slender trees in the foreground.\\
        \textbf{Art-style:} Art Nouveau (Modern).\\
        \textbf{Asymmetric balance} is evident in the composition, with the tall trees on the right balancing the expansive view of the water and islands on the left, creating a stable yet dynamic visual experience.\\
        \textbf{Harmony} is achieved through the consistent use of warm and cool colors, as well as the smooth transitions between the different elements of the landscape, creating a cohesive and unified composition.\\
        \textbf{Variety} is present in the different shapes and forms of the trees, islands, and hills, as well as the contrasting colors of the sky and water, adding visual interest without overwhelming the composition.\\
        \textbf{Unity} is evident in the composition through the consistent theme of the natural landscape, with all elements fitting together seamlessly to create a coherent and complete scene.\\
        \textbf{Contrast} is created by the dark silhouettes of the trees against the lighter background of the sky and water, drawing attention to the foreground and adding depth to the composition.\\
        \textbf{Emphasis} is placed on the tall trees in the foreground, which stand out due to their dark color and prominent position, guiding the viewer's eye through the composition.\\
        \textbf{Proportion} is maintained with the relative sizes of the trees, islands, and hills, creating a realistic sense of scale and depth in the composition.\\
        \textbf{Movement} is suggested by the gentle curves of the landscape and the flowing lines of the water, leading the viewer's eye across the composition in a smooth and calming manner.\\
        \textbf{Rhythm} is present in the repetition of the tree trunks and the undulating forms of the hills and islands, creating a sense of continuity and flow in the composition.
        }
        \end{subfigure}

        \begin{subfigure}{\linewidth}
        \includegraphics[width=\textwidth]{assets/artdapted_qualitative/combined_winston-churchill_woodland-scene-near-mimizan.jpg}
        \caption{}
        \parbox[t]{\linewidth}{
        \textbf{Prompt:} A forest scene with tall, slender trees casting long shadows on the ground.\\
        \textbf{Art-style:} Impressionism.\\
        \textbf{Asymmetric balance} is evident in the composition, with the trees distributed unevenly yet harmoniously across the scene, creating a natural and dynamic equilibrium.\\
        \textbf{Harmony} is achieved through the consistent use of green and brown tones, which unify the composition and create a cohesive forest scene.\\
        \textbf{Variety} is present in the different shapes and sizes of the trees, as well as the varying lengths and directions of the shadows, adding visual interest to the composition.\\
        \textbf{Unity} is evident as all elements in the composition, such as the trees and shadows, contribute to the overall theme of a forest, creating a coherent and complete scene.\\
        \textbf{Contrast} is present between the light and dark areas, particularly in the shadows cast by the trees, which adds depth and dimension to the composition.\\
        \textbf{Proportion} is maintained with the tall, slender trees dominating the composition, creating a sense of scale and depth that enhances the realism of the forest scene.\\
        \textbf{Movement} is suggested by the diagonal shadows and the slight lean of some trees, guiding the viewer's eyes through the forest and creating a sense of flow.\\
        \textbf{Rhythm} is created by the repetition of the tree trunks and the alternating light and shadow patterns on the ground, adding a sense of continuity and flow to the composition.\\
        \textbf{Pattern} is present in the regular spacing of the trees and the consistent direction of the shadows, contributing to the overall structure and order of the composition.}
        \end{subfigure}

        \begin{subfigure}{\linewidth}
        \includegraphics[width=\textwidth]{assets/artdapted_qualitative/combined_john-constable_the-hay-wain-1821.jpg}
        \caption{}
        \parbox[t]{\linewidth}{
        \textbf{Prompt:} A rural scene with a cottage, large trees, a river, a cart with a horse, and a dog in the foreground.\\
        \textbf{Art-style:} Romanticism.\\
        \textbf{Asymmetric balance} is evident in the composition, with the large trees and cottage on the left balanced by the open field and sky on the right, creating a sense of stability and equilibrium.\\
        \textbf{Harmony} is achieved through the cohesive use of natural elements and a consistent color palette, making the composition appear organized and unified.\\
        \textbf{Variety} is present in the different elements such as the cottage, trees, river, cart, and dog, adding interest and complexity to the composition.\\
        \textbf{Unity} is achieved by the consistent rural theme and the harmonious arrangement of elements, making the composition feel complete and coherent.\\
        \textbf{Contrast} is evident between the dark, dense foliage of the trees and the bright, open sky, highlighting the different aspects of the natural environment.\\
        \textbf{Emphasis} is placed on the cart and horse in the river, drawing attention to the human activity within the natural setting.\\
        \textbf{Proportion} is carefully considered, with the large trees and expansive sky creating a sense of depth and scale, enhancing the realism of the composition.\\
        \textbf{Movement} is suggested by the flowing river and the direction of the cart, guiding the viewer's eye through the composition.\\
        \textbf{Rhythm} is created by the repetition of natural elements such as trees and clouds, adding a sense of continuity and flow to the composition.}
        \end{subfigure}
    \end{multicols}
    \caption{ArtDapted generations based on the given prompt and art conditions.}
    \label{fig:compose-wise}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \scriptsize
%     \setlength{\tabcolsep}{0pt}
%     \begin{tabular}{c c c}
%     \begin{subfigure}{0.333\textwidth}
%         \includegraphics[width=\textwidth]{assets/artdapted_qualitative/combined_lawren-harris_afternoon-sun-lake-superior-1924.jpg}
%         \caption{}
%     \end{subfigure}&
%     \begin{subfigure}{0.333\textwidth}
%         \includegraphics[width=\textwidth]{assets/artdapted_qualitative/combined_winston-churchill_woodland-scene-near-mimizan.jpg}
%         \caption{}
%     \end{subfigure}&
%     \begin{subfigure}{0.333\textwidth}
%         \includegraphics[width=\textwidth]{assets/artdapted_qualitative/combined_john-constable_the-hay-wain-1821.jpg}
%         \caption{}
%     \end{subfigure}\\
%     \parbox[t]{.32\textwidth}{
    
%     }&
%     \parbox[t]{.32\textwidth}{
%     }&
%     \parbox[t]{.32\textwidth}{
%     }\\
%     \end{tabular}
%     \caption{}
% \end{figure}

==> fig/evaluation_piechart.tex <==
\begin{figure}[t]
    \centering
    % compart_winners_compart 501
    % compart_winners_artdapted 293
    % compart_winners_ella 96
    % compart_winners_baseline 110
    
    % winners_artdapted 577
    % winners_ella 188
    % winners_baseline 235
    \begin{tikzpicture}[every node/.style={font=\scriptsize}]
    \fill[blue] (0,0) rectangle (0,-1.8); % hack to vertical align pie chart with legend
    \pie[radius=1, rotate=90]{0/, 57.7/, 18.8/, 23.5/}
    \pie[pos={3,0}, radius=1, rotate=45, text=legend]{50.1/CompArt, 29.3/ArtDapter (Ours), 9.6/ELLA, 11/Baseline}
    \end{tikzpicture}
    \vspace{-2.5em}
    \caption{Evaluation results in terms of winning proportions of ArtDapter against baselines. Respectively, the left and right piechart correspond to two evaluation rounds where in the second, original CompArt images were also included in the judgment process.}
    \label{fig:evaluation_piechart}
\end{figure}

==> fig/principle_wise_cherry_picked.tex <==
\begin{figure}[H]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{p{0.2\textwidth} p{0.2\textwidth} p{0.2\textwidth} p{0.2\textwidth} p{0.2\textwidth}}
         \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/artdapted_ferdynand-ruszczyc_bajka-zimowa-1904_balance.jpg} & % balance
         \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/baseline_gustave-moreau_study-puff-adder_harmony.jpg} & % harmony
         \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/artdapted_abraham-manievich_untitled-1925_variety.jpg} & % variety
         \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/artdapted_camille-pissarro_the-banks-of-the-epte-at-eragny-1884_unity.jpg} & % unity
         \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/artdapted_armand-guillaumin_coucher-de-soleil-en-creuse-1898_contrast.jpg} \\ % contrast
        \parbox[t]{0.18\textwidth}{
        \textbf{Context}: A snowy forest scene with bare trees surrounding a dark, frozen pond.\\
        \textbf{Art-Style}: Post-Impressionism.\\
        \textbf{Symmetric balance} is evident in the composition, with the dark pond centrally placed and flanked by similar arrangements of snow-covered trees on both sides, creating a sense of equilibrium and stability.} &
        \parbox[t]{0.18\textwidth}{
        \textbf{Context}: A coiled snake with a detailed pattern on its body, depicted with a mix of brown, black, and yellow hues, against a plain background with handwritten text.\\
        \textbf{Art-Style}: Symbolism.\\
        \textbf{Harmony} is achieved through the consistent color palette of browns, blacks, and yellows, which unifies the snake with the background and text, creating a cohesive visual experience.} &
        \parbox[t]{0.18\textwidth}{
        \textbf{Context}: A vibrant scene of houses surrounded by trees with a colorful sky in the background.\\
        \textbf{Art-Style}: Expressionism.\\
        \textbf{Variety} is present in the diverse range of colors, shapes, and textures used throughout the composition, which engage the viewer and add visual interest and complexity.} &
        \parbox[t]{0.18\textwidth}{
        \textbf{Context}: A lush countryside scene with trees, a small pond, a house in the background, and cows grazing in the field.\\
        \textbf{Art-Style}: Impressionism.\\
        \textbf{Unity} is achieved by the consistent theme of a rural landscape, with all elements fitting together seamlessly to create a coherent and complete scene.} &
        \parbox[t]{0.18\textwidth}{
        \textbf{Context}: Landscape with rolling hills, a winding river, and ruins of a castle under a colorful sky.\\
        \textbf{Art-Style}: Impressionism.\\
        \textbf{Contrast} is created by the dark shadows of the hills and the bright colors of the sky, drawing attention to the different parts of the composition.} \\
         \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/artdapted_childe-hassam_blossoms-1883_emphasis.jpg} & \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/artdapted_nicholas-roerich_ladakh-1937_proportion.jpg} & \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/artdapted_alfred-sisley_cow-pasture-near-louveciennes-1875_movement.jpg} & \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/baseline_gustave-courbet_the-wave-1871_rhythm.jpg} & \includegraphics[width=.2\textwidth,height=.2\textwidth]{assets/artdapted_john-henry-twachtman_greenwich-garden-1899_pattern.jpg} \\
        \parbox[t]{.18\textwidth}{
        \textbf{Context}: A landscape with blooming trees and a grassy foreground under a blue sky.\\
        \textbf{Art-Style}: Impressionism\\
        \textbf{Emphasis} is placed on the blooming trees, which are the focal point of the composition due to their central placement and vibrant colors.} &
        \parbox[t]{.18\textwidth}{
        \textbf{Context}: Mountainous landscape with layered hills and silhouettes of structures in the foreground and background under a cloudy sky.\\
        \textbf{Art-Style}: Symoblism.\\
        \textbf{Proportion} is used to create a sense of depth, with larger structures in the foreground and smaller, more distant mountains in the background, enhancing the three-dimensionality of the composition.} &
        \parbox[t]{.18\textwidth}{
        \textbf{Context}: A pastoral scene with a woman standing by a tree, cows grazing, and a winding path leading through a lush green landscape under a partly cloudy sky.\\
        \textbf{Art-Style}: Impressionism.\\
        \textbf{Movement} is suggested by the winding path leading the viewer's eye through the landscape, creating a gentle flow and guiding the gaze across the composition.} &
        \parbox[t]{.18\textwidth}{
        \textbf{Context}: A stormy seascape with crashing waves and rocks on the shore under a cloudy sky.\\
        \textbf{Art-Style}: Realism.\\
        \textbf{Rhythm} is present in the repetitive patterns of the waves and the clouds, creating a sense of continuity and flow in the composition.} &
        \parbox[t]{.18\textwidth}{
        \textbf{Context}: A lush garden with abundant white flowers and green foliage, with a body of water and trees in the background.\\
        \textbf{Art-Style}: Impressionism.\\
        \textbf{Pattern} is present in the consistent arrangement of the flowers and leaves, adding a sense of order and structure to the composition while enhancing its visual appeal.} \\
    \end{tabular}
    \caption{Images generated by ArtDapter in accordance to the specified art controls.}
    \labauxfig{fig:principle-wise-cherry-picked}
\end{figure}

==> fig/results.tex <==
\begin{figure}[t]
    % \showlinewidth
    \definecolor{clr1}{RGB}{178, 190, 195}
    \definecolor{clr2}{RGB}{162, 155, 254}
    \definecolor{clr3}{RGB}{255, 118, 117}
    \definecolor{clr4}{RGB}{116, 185, 255}
    \input{fig/scorecard_example}%
    % Right column with two stacked subfigures
    \begin{minipage}[t]{0.5\linewidth}
        \input{fig/results_principle_level}
        \input{fig/results_composition_level}
    \end{minipage}
    \caption{Example evaluation scorecard (a) and evaluation results (b,c). Evaluation is assessed at both principle and composition levels, reporting each model's winning percentages. For each level, the results for ASSMT and ASSMT* assessments are respectively reported in its top and bottom subplots. Crucially, the only difference between the assessment rounds is that for ASSMT*, original CompArt artworks were also included in the judgment process.}
    \label{results}
\end{figure}

% GPT is instructed to score on the 7-point Likert Scale~\cite{likert1932measurement} with 1 being poor alignment and 7 being excellent alignment. The GPT prompt used is included in the Supplementary Materials~\cref{sec:evaluation_prompt}. The IR scoring prompt is obtained by concatenating the caption with the PoA condition in question. To decide the winner of each PoA condition alignment, we simply pick the image with the highest GPT score. If there is a tie, the one with higher IR score is chosen. The overall winner for the generation is the image with the most PoA alignment wins. For the given example, if CompArt was included in the evaluation round, then it is the overall winner with 5 PoA alignment wins. If we did not include CompArt, then the overall winner is ArtDapter with 9 PoA alignment wins.

==> sec/auxiliary_materials.tex <==
\appendix
\clearpage
\onecolumn
% \appendixmargins{22mm}{22mm}{24mm}{24mm}
% \crefname{appendix}{Section}{Sections}
% \Crefname{appendix}{Section}{Sections}
% \crefname{auxfigure}{Figure}{Figures}
% \Crefname{auxfigure}{Figure}{Figures}

\begin{center}
    {\Large \textbf{Auxiliary Materials}}
\end{center}

\textit{The Auxiliary Materials present our Principles of Art definitions, the GPT-4o prompts used and additional qualitative analysis on GPT-4o and our model.}

\startcontents[aux] % start collecting appendix-only TOC entries
\section*{Contents}
\begingroup
  \setcounter{tocdepth}{2}% show \section and \subsection
  \printcontents[aux]{l}{1}{}% “l” = use the class’ \l@section, \l@subsection, etc.
\endgroup

\section{Principles of Art}
\label{sec:PoA}
The Principles of Art (PoA) is a set of guidelines for composing artworks. The elements used for composition are known as the elements of art (EoA), which generally comprise line, shape, texture, form, space, colour and value. The PoA can be used in any number of ways to achieve visual storytelling: arousing interest, evoking feelings or conveying certain ideas to viewers. It also provides viewers with a framework to analyse, appreciate and reason about artworks from a compositional perspective. PoA are not mutually exclusive to one another as they are intricately related concepts. We shall define each PoA in the following 10 paragraphs. For each principle, we attempt to answer the following questions in order, ``What is it about?'', ``What effect(s) does it bring to a composition?'', ``How can it be brought about in the composition?'', ``What does a lack of it bring to the composition?'', ``What does an excess of it bring to the composition?'', ``How does it relate to other PoA?''.
\begin{enumerate}
    \item \textbf{Balance} is the distribution of visual weight in the composition. The objects being balanced can be visual elements or EoA. Balance brings a sense of equilibrium and stability to the composition by ensuring no one part overpowers another. Balance can be achieved through (1) symmetrical balance about an axis with both sides being identical or nearly identical, (2) asymmetrical balance about an axis with both sides comprising different elements but sharing similar visual weight, or (3) radial balance about a point with objects radiating outwards from or encircling around it. Unbalanced compositions can appear unfinished, unsettling and distract viewers from the intended messages. Overly-balanced compositions can appear predictable and monotonous, lacking dynamism and interest. Balance often works with harmony to create a cohesive and stable composition. It also works with contrast and emphasis when ensuring that focal points are highlighted without overwhelming the composition.
    \item \textbf{Harmony} is the state of cohesiveness in the composition where all parts contribute to the whole by appearing coordinated. Harmony brings a sense of order and cohesiveness, making the composition appear organised. It usually also brings about coherence and unity. It is achieved via the uniformity of different parts in the composition. Uniformity can come from a consistency in EoA employed or from other salient regularities such as analogous colour schemes. Insufficient harmony with excessive variety can make the composition appear uncoordinated and haphazard. Excessive harmony with insufficient variety and contrast can make the composition appear flat and predictable. Harmony is closely related to unity as cohesiveness often also elevates coherence in the composition. Harmony also relates to balance as cohesiveness and stability are closely intertwined. Harmony often opposes variety and therefore works with it in managing visual interest without introducing chaos.
    \item \textbf{Variety} is the diversity and complexity of visual elements in the composition. Variety engages the viewer and holds their attention by creating regions of visual interest for exploration. It also brings excitement and dynamism to the composition. Variety can be achieved by varying either EoA employed or other visual attributes such as proportions and placements. Insufficient variety can make the composition appear monotonous and repetitive. Excessive variety may cause the composition to appear chaotic with too many elements fighting for attention. Variety can oppose harmony so the two work closely to ensure that the composition is interesting yet cohesive. Variety also contributes towards contrast and emphasis when differences are highlighted.
    \item \textbf{Unity} is the state of coherence or oneness, where all elements fit into the composition without appearing forced or out-of-place. Unity brings coherence to the composition by presenting elements which align well with one's expectations (e.g. a fruits basket containing only fruits). It also brings a sense of completeness when most of what's expected is present (e.g. a round table with chairs around it). By intentionally leaving out an expected element, unity can also be manipulated to highlight the absence of it (e.g. a family portrait without a father figure). Unity can be achieved when different parts of the composition adhere to a clear context, theme or message. The adherence can come from a consistency in EoA employed, a repetition of visual elements, a unified colour scheme, a recurring motif or simply semantic relevance. Insufficient unity can make the composition appear confusing, disjoint, and fragmented with superfluous parts. Excessive unity and harmony can suppress variety, create monotony and appear too predictable, lowering visual engagement. Unity is often enhanced by harmony and the two are closely related. Unity can also be realised through balance, proportion and rhythm. An element that is not unified with the composition stands out and can therefore bring emphasis to itself.
    \item \textbf{Contrast} is the use of opposing visual elements in the composition. Contrast brings drama, excitement and focus to the composition, highlighting differences and drawing attention to important areas. Contrast can be achieved through the use of contrasting EoA and the juxtapositions of opposing visual elements. Insufficient contrast can make the composition appear flat, lacking focus points and leaving little visual impression. Excessive contrast can make the composition appear jarring, disjointed and overwhelming. Contrast is often employed for emphasis and they work with balance to ensure that focal points are highlighted without overpowering the composition. Contrast is usually directly correlated with variety. Contrast can also create movement by guiding the eyes across the composition.
    \item \textbf{Emphasis} is the presence of focal points within the composition which draw attention to its important parts. Emphasis helps communicate the intended message effectively by bringing focus and interest to the main subjects and prominent areas in the composition. These areas tend to be the first (and perhaps also the last) regions to be gazed at. Emphasis can be created via stark contrasts, placement in prominent positions (e.g. centre or foreground), converging lines, isolation from other visual elements, exaggerated proportions and the use of variety to highlight specific areas. Insufficient emphasis can make the composition appear monotonous and directionless, with no clear regions of interest. Excessive emphasis can create too many focal points, leading to confusion and a lack of clear focus. Emphasis often works with contrast to highlight important areas. It also works with balance when focal points are emphasised without overwhelming the composition. With multiple regions of emphasis, movement is also created by guiding the eyes across the composition.
    \item \textbf{Proportion} is the sense of scale and depth from the relative sizes between visual elements in the composition. Proportion influences viewers' perception and interpretation by manipulating depth and perspective in the composition. Relative sizes between visual elements can describe their relationship and importance. The presence of specific ratios and principles (e.g. the golden ratio) can also enhance aesthetics. Proportion can be achieved by carefully considering the size and scale of visual elements. For example, related visual elements can possess similar sizes while important elements can overpower surrounding elements in terms of scale. Realistic proportions help achieve realism while exaggerated and distorted proportions can be employed for artistic effect. Insufficient proportion can damage balance and harmony, make the composition appear too unrealistic or create excessive visual distortion and confuse viewers. Excessive proportion can lead to a lack of variety and interest, making the composition appear repetitive. Proportion often works with balance to ensure visual elements are balanced by their sizes. Consistent and appropriate sizing of visual elements also ensure a cohesive and coherent composition, contributing to harmony and unity. Proportion also creates emphasis by highlighting specific areas through size and scale.
    \item \textbf{Movement} is the appearance or suggestion of motions within the composition. Movement facilitates visual narration by guiding the eyes in the composition. It adds dynamism and flow to a still composition, making it appear alive and engaging. It can also create tension via the anticipation of unfolding events in the scene. Movement can be created by the repetition of EoA suggesting directions or rhythmic motions (e.g. diagonal/converging lines, swirling curves), implied by the arrangement of elements depicting motion and direction (e.g. objects falling off an edge), or introduced by scenes that lead the gaze (e.g. a flowing river, human traffic). It can also be achieved by some optical illusions. Insufficient movement can make the composition appear static, lifeless, and unengaging. Excessive movement can create chaos and confusion, distracting viewers from important aspects. Movement often works with rhythm and pattern when creating a smooth, rhythmic and continuous sense of flow. Contrast and emphasis can work with movement to create sequential navigational points for the eyes (e.g. The Scream by Edvard Munch).
    \item \textbf{Rhythm} is the presence of visual tempo in the composition. Rhythm adds a sense of continuity, flow and dynamism to the composition. It can also help blend and connect distinct parts together in a cohesive manner (e.g. trees connected via bushes). Visual tempo can be manipulated to evoke either calmness (e.g. grass on a windy field) or excitement (e.g. crashing waves). Rhythm is achieved by the continuous repetition, sequential progression (e.g. gradual increment) or alternation (e.g. varying the spacing or arrangement at intervals) of EoA or visual elements. Insufficient rhythm can make the composition appear sparse and static. Excessive rhythm can make the composition appear repetitive and monotonous. Rhythm introduces movement through flow, and variety through visual tempo. It also elevates harmony and unity when it blends different visual elements together cohesively and coherently.
    \item \textbf{Pattern} is the repetition of elements in a consistent and organised manner within the composition. Patterns are often decorative and add texture and visual appeal to the composition, increasing its visual engagement. Their repetitive nature can bring a sense of predictability, order and structure to the composition. Pattern also creates a discrete sense of movement and flow. Pattern is sometimes used to create emphasis via the strategic placement of irregularities. Patterns can be simple through the consistent repetition of EoA or complex by combining and arranging elements (e.g. motifs or designs) in a regular and consistent manner. Insufficient pattern can make the composition appear chaotic and disorganised. Excessive pattern can introduce rigidity and predictability, making the composition appear static and monotonous. Pattern is more rigid than rhythm but they are closely related as their techniques overlap. Pattern directly relates to variety, with more complex patterns corresponding to higher variety. It also relates to harmony and unity when arranging elements in a cohesive and coherent manner. Patterns are often themselves balanced by construction.
\end{enumerate}

\newpage
\section{CompArt annotation}
\label{sec:compart_annotation}
\subsection{Specification}
The original WikiArt dataset comes with artwork images annotated with their artist name, art style and art genre. Using GPT-4o, we further annotate each example with a caption, a compositional analysis in terms of PoA and also its ranked top 3 predicted art-styles. The art-style prediction serves to provide us with an indicator of the MLLM's artistic knowledge. Crucially, we instructed the MLLM to obey the following rules and formats during annotation:

\textbf{Captions} are to be concise and objective about the artwork's contents. They cannot mention the image being an artwork as they serve to only provide the context for generation. This is a heuristic to leverage on the existing generalisability of the pre-trained T2I model and maximize the sensitivity of the ArtDapter in adhering to artistic controls.

\textbf{Compositional analysis} needs to strictly accord to the 10 PoA we defined. For each PoA, a prominence level on the scale [weak, mild, moderate, strong] is to be indicated. Analysis for a principle with a weak prominence is optional. Otherwise, the analysis must provide a concise and high-quality analysis on \textit{where} in the composition is the principle evident, \textit{which} visual elements are involved, \textit{how} the principle is achieved and \textit{what} are its intended effects. For analysis on balance principle, the specified balance type must be ``symmetric'', ``asymmetric'' or ``radial''. To ensure reporting consistency, the first sentence's subject for every analysis must be the principle being analyzed. Lastly, the artwork should only be referred to as ``the composition''. This is to prevent the mixing of art-style and medium (e.g. ``the oil painting'') into the compositional analysis.

\subsection{Prompt}
\label{sec:annotation_prompt}
The following is the prompt used for instructing the MLLM to annotate each and every artwork in WikiArt. Note that definition of each PoA in the prompt accord exactly as per \cref{sec:PoA} and is truncated here for brevity.
\begin{tcolorbox}[left=1pt,right=1pt,top=1pt,bottom=1pt, breakable,enhanced]
\footnotesize
The Principles of Art (PoA) is a set of guidelines for composing artworks. The elements used for composition are known as the elements of art (EoA), which generally comprise line, shape, texture, form, space, colour and value. The PoA can be used in any number of ways to achieve visual storytelling: arousing interest, evoking feelings or conveying certain ideas to viewers. It also provides viewers with a framework to analyse, appreciate and reason about artworks from a compositional perspective. PoA are not mutually exclusive to one another as they are intricately related concepts. We shall define each PoA in the following 10 paragraphs.\\

1. Balance is the ...\\
2. Harmony is the ...\\
3. Variety is the ...\\
4. Unity is the ...\\
5. Contrast is the ...\\
6. Emphasis is the ...\\
7. Proportion is the ...\\
8. Movement is the ...\\
9. Rhythm is the ...\\
10. Pattern is the ...\\

Now act as an expert art analyst. Given an artwork image, please accomplish 3 tasks:\\

1. Present a concise and objective caption about the artwork's contents and avoid any mention of the image being an artwork. Do not start with "The".\\
2. Identify the primary style of the artwork strictly from the categories [Post-Impressionism, Expressionism, Impressionism, Northern Renaissance, Realism, Romanticism, Symbolism, Art Nouveau (Modern), Naïve Art (Primitivism), Baroque, Rococo, Abstract Expressionism, Cubism, Color Field Painting, Pop Art, Pointillism, Early Renaissance, Ukiyo-e, Mannerism (Late Renaissance), High Renaissance, Fauvism, Minimalism, Action painting, Contemporary Realism, Synthetic Cubism, New Realism, Analytical Cubism]. Provide the top-3 most likely styles, ordered from most to least confident.\\
3. Present a compositional study of the artwork according to the 10 PoA we defined. If a principle is present, indicate a prominence level on the scale [weak, mild, moderate, strong]. For weak, no analysis is needed. Otherwise, provide a concise and high-quality analysis on the locations in the composition where the principle is evident, the visual elements or EoA involved, how the principle is achieved and its intended effects. For analysis on balance principle, specify the balance type [symmetric, asymmetric, radial] present. For each analysis: the first sentence's subject must be the principle being analysed (e.g. 'Asymmetric balance is evident...'); refer to the artwork only as "the composition".\\

Output in the following JSON format:
\begin{verbatim}
{
  "caption": <caption>,
  "style": [<style 1>, <style 2>, <style 3>],
  "PoA": {
    "balance": {
      "prominence": <prominence>,
      "analysis": <analysis>
    },
    ...
  }
}
\end{verbatim}
\end{tcolorbox}

\newpage
\section{Evaluation}
\subsection{Prompt}
\label{sec:evaluation_prompt}
This details the prompt structure used for evaluation of ArtDapted outputs against baselines. Note that the \textit{evaluation statements} in the prompt would differ for every test example. For the sake of brevity, they are truncated in the following example. Alike \cref{sec:annotation_prompt}, the definition of each PoA in the prompt accord exactly as per \cref{sec:PoA} and is also truncated here for brevity.
\begin{tcolorbox}[left=1pt,right=1pt,top=1pt,bottom=1pt, breakable,enhanced]
\footnotesize
The Principles of Art (PoA) is a set of guidelines for composing artworks. The elements used for composition are known as the elements of art (EoA), which generally comprise line, shape, texture, form, space, colour and value. The PoA can be used in any number of ways to achieve visual storytelling: arousing interest, evoking feelings or conveying certain ideas to viewers. It also provides viewers with a framework to analyse, appreciate and reason about artworks from a compositional perspective. PoA are not mutually exclusive to one another as they are intricately related concepts. We shall define each PoA in the following 10 paragraphs.\\

1. Balance is the ...\\
2. Harmony is the ...\\
3. Variety is the ...\\
4. Unity is the ...\\
5. Contrast is the ...\\
6. Emphasis is the ...\\
7. Proportion is the ...\\
8. Movement is the ...\\
9. Rhythm is the ...\\
10. Pattern is the ...\\

EVALUATION STATEMENTS\\

The following lines are evaluation statements specifying image content and PoA analysis. Each line is in the format of \textlangle statement type\textrangle: \textlangle statement\textrangle.
\textbf{content}: A winged horse carrying a man and a woman, with the woman clinging to the man as they ascend from a cliff.\\
\textbf{balance}: Asymmetric balance is evident ...\\
\textbf{variety}: Variety is present in the ...\\
\textbf{unity}: Unity is evident as all elements...\\
\textbf{contrast}: Contrast is created through...\\
\textbf{emphasis}: Emphasis is placed on the...\\
\textbf{proportion}: Proportion is maintained with the...\\
\textbf{movement}: Movement is suggested by the...\\

EVALUATION INSTRUCTIONS\\

Now act as an expert art analyst based on the 10 PoA we defined. For every image provided, you are to score how well each of the evaluation statements is represented in the image. Scoring is done on the seven-point Likert Scale (1 = Poor representation, 7 = Excellent representation). Output a list in the sequence of provided images where each item reports the scores for the corresponding image. The scores for a particular image is captured by a dictionary of \textlangle statement type\textrangle: \textlangle score\textrangle~key-value pairs. Do not report any statement types not in the evaluation statements. Output in strict JSON format like the following example:
\begin{verbatim}
{
  "results": [
    {
      "content": 7,
      "balance": 6,
      "harmony": 6,
      ...
    },
    {
      "content": 7,
      "balance": 6,
      "harmony": 5,
      ...
    },
    {
      "content": 5,
      "balance": 5,
      "harmony": 4,
      ...
    },
    {
      "content": 7,
      "balance": 6,
      "harmony": 1,
      ...
    }
  ]
}}
\end{verbatim}

\end{tcolorbox}

\newpage
\section{Additional analyses}

\subsection{GPT-4o}
\label{sec:gpt4o-qualitative}
\input{fig/gpt4o_qualitative}

In this section we attempt to qualitatively assess the capabilities of GPT-4o in understanding art. We first point out the relevant limitations of GPT-4o as officially stated by OpenAI at the time of this work\footnote{\url{https://platform.openai.com/docs/guides/vision}}. Crucially, the MLLM might misinterpret rotated images, fail at counting objects in the image and struggle with spatial reasoning which concerns precise object localization in the image. In addition, images are resized before analysis and this implies that original proportions are not preserved and certain intentional proportions might not be correctly interpreted by the model.

Despite the above limitations, we found GPT-4o to display strong artistic comprehension ability. Given how art often express concepts through abstract and creative means such as motifs, patterns and styles, art-comprehension is particularly challenging, even to humans. To the best of our knowledge, no works in the literature has attempted to assess MLLMs in this challenging domain. To gather some sense of GPT-4o's capability, we established a simple test by requesting it to describe 8 challenging handpicked images we curated from the internet. We report GPT's responses in \cref{fig:gpt4o-qualitative}.

Notably, \cref{fig:girl_with_a_pearl_earring,fig:rethink_plastic,fig:mona_lisa,fig:starry_night_on_a_pcb} respectively are based off ``Girl with a Pearl Earring'' by Johannes Vermeer, ``The
Thinker'' by Auguste Rodin, ``Mona Lisa'' by Leonardo da Vinci and ``Starry Night'' by Vincent van Gogh. In addition to assessing whether the MLLM can ``perceive'' past the visual abstractions, these images are also a test of the MLLM's knowledge of art since the references in question are of famous artworks. On all images except~\cref{fig:mona_lisa}, GPT-4o correctly identified their references, explaining how salient artistic motifs are recreated along the way. Impressively, GPT-4o's response on~\cref{fig:rethink_plastic} also correctly inferred the social commentary the artwork is making on plastic waste, without being provided the context of the artwork's actual title ``Rethink Plastic''. Interestingly, we found that despite GPT-4o not mentioning Mona Lisa on its first reply, it was able to correctly identify it in subsequent replies when pressed for an artistic reference. This suggests that while GPT-4o has the capability for abstract visual reasoning, some prompt tuning is perhaps needed to draw it out.

\cref{fig:mona_lisa,fig:penny_dreadful,fig:aquarium,fig:eyes,fig:sink_draining} serve to test the MLLM's ability to recognize and explain optical illusions across different styles. On all images except~\cref{fig:mona_lisa,fig:penny_dreadful}, GPT-4o correctly identified the optical illusions at play and their intended effects. \cref{fig:mona_lisa} was the failure case on Mona Lisa as previously explained. \cref{fig:penny_dreadful} presents the impression of a screaming skull face that was not picked by GPT-4o. In \cref{fig:aquarium}, GPT-4o guessed that the vertical line was a ``wall or a barrier'' which suggests that it did not identify the fish to be inside a tank. However, it did correctly interpret the cat's eye to be depicted as the fish, which is perhaps a more challenging interpretation than the fish tank. In \cref{fig:eyes}, GPT-4o understood the motif of eyes but the pair of red eyes was interpreted to be in the center of the image as opposed to being situated some distance South-West from the center. This could be due to a combination of resizing and the spatial reasoning limitations of the model. It also did not mention that the gaze of all the eyes converges on the pair of red eyes. GPT-4o did however, correctly identify the abstract representation of eyes and the intention of the pair of red eyes to draw visual attention by serving as the focal point of the composition. Most impressive was its response on~\cref{fig:sink_draining}, where it correctly identified the image to capture a draining sink which creates the impression of an eye.

It is important to note that we carried out this above test using OpenAI's API endpoint which receives the images in Base64 text encoded format, without filenames. In our tests, we have found that GPT's web chat application can make use of uploaded image filenames for additional contextual clues.

We also point out some problems we have noticed with GPT-4o's annotations in our CompArt dataset, which we exhibit in \cref{fig:compart-qualitative-issues}. Since the PoA principle of balance is the most prevalent annotation in the dataset and also the most encompassing in terms of spatial relations, we shall analyze along this dimension. Firstly, GPT-4o's understanding of symmetric and asymmetric balance is found to be inconsistent across some artworks. All \cref{fig:francisco-goya_the-duke-of-osuna-and-his-family-1788,fig:orest-kiprensky_portrait-of-a-military-doctor-1812,fig:giovanni-bellini_madonna-and-child-1490} were annotated with symmetric balance but did not display strict major axes of reflection. While \cref{fig:giovanni-bellini_madonna-and-child-1490} displays a more salient vertical axis of reflection due to the background pillar, the visual weight of the woman on the left is significantly heavier than the infant on the right. By GPT-4o's symmetry standards of these 3 examples, one would expect \cref{fig:joshua-reynolds_frederick-howard-5th-earl-of-carlisle} to also be understood to exhibit symmetrical balance but was instead annotated to be asymmetric. We are unsure if these inconsistencies are hallucinatory in nature or due to ambiguities in our prompt, or both. We notice that GPT-4o is also biased towards establishing balance in terms of left and right when the more salient balance is top-bottom (i.e. horizontal axis). Such is observed in \cref{fig:boris-kustodiev_in-the-box-1912,fig:compart_qualitative/odilon-redon_the-angel-of-destiny}. In addition, \cref{fig:compart_qualitative/lorenzo-lotto_allegory-of-chastity-1505} displays both strong vertical and horizontal axes of symmetry but only the left-right balance was identified, forcing the cherub at the top to be assigned to the left-half and the woman at the bottom to be assigned to the right-half even though they are clearly intended to be positioned along the central vertical axis. Moreover, sometimes the notions of left and right are muddled like in \cref{fig:boris-kustodiev_in-the-box-1912,fig:bartolome-esteban-murillo_adoration-of-the-shepherds-1} or even have their definitions completely swapped as observed in \cref{fig:gustav-klimt_roses-under-the-tree}. Finally, where numeration are involved, the annotations suffer from miscounting as seen in \cref{fig:koloman-moser_picture-book-for-the-niece-of-ditha-mautner-von-markhof-1904-3} where the eight cats were wrongly counted as ``seven dogs''. This is consistent with the limitations of GPT-4o as officially stated by OpenAI.

\input{fig/compart_qualitative_issues}

\newpage
\subsection{CompArt}
\input{fig/compart_style_wise_principle_wise}
\input{fig/word_clouds}

\newpage
\input{fig/compose_wise}
\newpage
\subsection{ArtDapter}
\label{sec:artdapter_qualitative}
Here we attempt to provide some qualitative analysis of ArtDapter's capabilities and limitations.

We first assess the capabilities of our ArtDapted model in composing multiple PoA controls together in a single generation. This is exhibited in \cref{fig:compose-wise}. We also attempt to perceive how our ArtDapted model perform on each PoA principle individually (i.e. without composing multiple PoA conditions at the same time). A principle-wise collage of different generations is presented in \cref{fig:teaser}. In addition, we also study the generations across different PoA controls while keeping the prompt and art-style fixed. This is reported in \cref{fig:principle-wise}. From the examples it suggests that our ArtDapted model is capable of both composing multiple PoA controls in a joint manner while also retaining the ability to respect the controls specified by each individual principle.

Additionally, in \cref{fig:style-wise}, we explore ArtDapter's learnt understanding of art-style by varying the art-style while keeping the PoA controls fixed. Interestingly, it appears that our model attaches more high-frequency details and colour balance to the notion of art-style. We also observe that it takes a combination of certain keywords in the prompt and PoA along with the art-style to produce a specific artistic motif. For instance, \cref{fig:style-wise} demonstrates that it is only with the ``Post-Impressionism'' art-style and the keyword ``swirling'' in the prompt and PoA controls that encourages our model to generate outputs with the motifs of Vincent van Gogh, the renowned Dutch Post-Impressionist painter. This is indicative that through our training scheme, high-level artistic motifs are decomposed down to a level that can be captured by compositional and art-style specifications.

The model is of course not without limitations. We observe that semantic alignment can sometimes fail with the generated output either omitting certain content or disrespecting certain constraints entirely. For example, in \cref{fig:teaser}, the symmetry balance-conditioned output did not include any ``dark frozen pond.'', the harmony-conditioned output did not include brown hues, the unity-conditioned output did not contain a house in the background and the contrast-conditioned output didn't not include the ruins of a castle. We have also observed object localization and numeration issues also evident in the dataset. Moreover, image fidelity are sometimes also low, with animals and human faces being un-artistically distorted or failing to adhere to the overall realism of the scene.
\clearpage
\input{fig/style_wise}
\input{fig/principle_wise}

\stopcontents[aux]

\papermargins % go back to the llncs defaults

==> tab/analysis.tex <==
\begin{table}
    \centering
    \tiny
    \caption{Overall caption for both subtables}
    \input{tab/linguistic_analysis}
    \label{tab:analysis}
\end{table}

